A two-stage estimation procedure for non-linear structural equation models

Applications of structural equation models (SEMs) are often restricted to linear associations between variables. Maximum likelihood (ML) estimation in non-linear models may be complex and require numerical integration. Furthermore, ML inference is sensitive to distributional assumptions. In this paper, we introduce a simple two-stage estimation technique for estimation of non-linear associations between latent variables. Here both steps are based on fitting linear SEMs: first a linear model is fitted to data on the latent predictor and terms describing the non-linear effect are predicted by their conditional means. In the second step, the predictions are included in a linear model for the latent outcome variable. We show that this procedure is consistent and identifies its asymptotic distribution. We also illustrate how this framework easily allows the association between latent variables to be modelled using restricted cubic splines and we develop a modified estimator which is robust to non-normality of the latent predictor. In a simulation study, we compare the proposed method to MLE and alternative two-stage estimation techniques.

==> integralform.tex <==
\section{Detailed derivations of integral formulas in section 3}
\label{sec:app:integralform}

We start by equation (\ref{ns1}) used for estimation of
natural cubic splines: \(\E[(\xi_{i}-t_j)^3 1_{\xi_{i}>t_j}\vert X_i, Z_i]= \int_0^\infty v^3
\frac{1}{\sqrt{2\pi} s}\exp(-\frac{(v-\mu)^2}{2 s^2})dv,\)
where \(V= \xi_{i}-t_j\), and \(V\sim N(\mu, s^2)\) with \(\mu=m_{x,z}-t_{j}\). Following a change of variable
(\(y=\frac{v-\mu}{s}\)) and
rewriting the polynomial using the binomial sum, the integral becomes
\begin{eqnarray}\label{cubicsum}
  \begin{array}{l}
    \frac{1}{\sqrt{2 \pi}} \int_{-\mu/s}^{\infty} (\mu + ys)^3
    \exp(-y^2/2) dy  =
    \frac{1}{\sqrt{2 \pi}} \sum_{k=0}^3 \left( \begin{array}{c} 3 \\ k \end{array}
    \right) \mu^{3-k} s^k \int_{-\mu/s}^{\infty} y^k
    \exp(-y^2/2)dy
  \end{array}
\end{eqnarray}

Now it is straight forward to see \(\int_{-\mu/s}^{\infty} \exp(-y^2/2) dy= \sqrt{2 \pi}
[1-\Phi(\frac{-\mu}{s})]\) and using integration by parts we have

\begin{enumerate}
\item \(\int_{-\mu/s}^{\infty} y \exp(-y^2/2) dy =
[-\exp(-y^2/2)]_{-\mu/s}^{\infty}=
\exp(-[\frac{\mu}{s \sqrt{2}}]^2)\)


\item \(\int_{-\mu/s}^{\infty} y^2 \exp(-y^2/2) dy = [-y
\exp(-y^2/2)]_{-\mu/s}^{\infty} + \int_{-\mu/s}^{\infty} \exp(-y^2/2)
dy =  \frac{-\mu}{s} \exp(-[\frac{\mu}{s \sqrt{2}}]^2) +  \sqrt{2 \pi}
[1-\Phi(\frac{-\mu}{s})]\)

\item \(\int_{-\mu/s}^{\infty} y^3 \exp(-y^2/2) dy= [-y^2
\exp(-y^2/2)]_{-\mu/s}^{\infty} + \int_{-\mu/s}^{\infty} 2 y \exp(-y^2/2)
dy = \frac{\mu^2}{s^2} \exp(-[\frac{\mu}{s \sqrt{2}}]^2) +  2 \exp(-[\frac{\mu}{s \sqrt{2}}]^2)\)
\end{enumerate}

The sum (\ref{cubicsum}) becomes
\begin{align*}
\E[(\xi_{i}-t_j)^3 1_{\xi_{i}>t_j}\vert X_i,
Z_i]=\exp(-[\frac{\mu}{s \sqrt{2}}]^2) \frac{s}{\sqrt{2 \pi}}
(\mu^2+2s^2)+ (\mu^3+ 3\mu s^2)[1-\Phi(\frac{-\mu}{s})]  
\end{align*}
which is the same as the expression (\ref{ns1}) because 
\(p_{x,z,j}=P(\xi_{i}>t_j \vert X_i, Z_i)=1-\Phi( \frac{-\mu}{s})\).\\

From the above calculations, expressions (\ref{special})  follow immediately, i.e.,
\begin{eqnarray*}\label{sp2}
 \begin{array}{lcl}
\E[(\xi_{i}-t_j) 1_{\xi_{i}>t_j}\vert X_i, Z_i]& = & \mu \int_{-\mu/s}^{\infty}
\frac{1}{\sqrt{2\pi}} \exp(-y^2/2) dy + \frac{1}{\sqrt{2\pi}} s
\int_{-\mu/s}^{\infty} \exp(-y^2/2) dy  \\
 & = & \mu [1-\Phi(\frac{-\mu}{s})] + s \frac{1}{\sqrt{2\pi}}
\exp(-[\frac{\mu}{s \sqrt{2}}]^2)
\end{array}
    \end{eqnarray*}
and 
\begin{eqnarray*}\label{sp3}
  \begin{array}{lcl}
    \E(\xi_i 1_{\{\xi_i < \tau\}}\vert X_i, Z_i) & = & \int_{\infty}^0 v
                                            \frac{1}{\sqrt{2\pi} s}\exp(-\frac{(v-\mu)^2}{2 s^2})dv\\
                                      &=&
                                          \int_{-\infty}^{-\mu/s} (\mu + sy) \exp(-y^2/2) dy\\
                                      &=& \mu
                                          \int_{-\infty}^{-\mu/s} \frac{1}{\sqrt{2\pi}} \mu \exp(-y^2/2) dy +\frac{s}{\sqrt{2\pi}} \int_{-\infty}^{-\mu/s} y \exp(-y^2/2) dy\\
                                      & = & \mu \Phi(\frac{-\mu}{s}) - \frac{s}{\sqrt{2\pi}} \exp(-[\frac{\mu}{s \sqrt{2}}]^2)
  \end{array}
\end{eqnarray*}

